MEC-aware Cell Association for 5G Heterogeneous Networks

The need for efficient use of network resources is continuously increasing with the grow of traffic demand, however, current mobile systems have been planned and deployed so far with the mere aim of enhancing radio coverage and capacity. Unfortunately, this approach is not sustainable anymore, as 5G communication systems will have to cope with huge amounts of traffic, heterogeneous in terms of latency among other Qualityof- Service (QoS) requirements. Moreover, the advent of Multiaccess Edge Computing (MEC) brings up the need to more efficiently plan and dimension network deployment by means of jointly exploiting the available radio and processing resources. From this standpoint, advanced cell association of users can play a key role for 5G systems. Focusing on a Heterogeneous Network (HetNet), this paper proposes a comparison between state-of-the-art (i.e., radio-only) and MEC-aware cell association rules, taking the scenario of task offloading in the Uplink (UL) as an example. Numerical evaluations show that the proposed cell association rule provides nearly 60% latency reduction, as compared to its standard, radio-exclusive counterpart.

==> simulation_results/figures/PDB_CCDF/PDB_CCDF.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
%

 \resizebox {\columnwidth} {!} {
 	
\begin{tikzpicture}

\begin{axis}[%
width==0.9*7cm,
height==0.9*7cm,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=1,
xlabel style={font=\color{white!15!black}},
xlabel={PBD Threshold [Sec]},
ymin=0.2,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$ \mathbb{P}\;\text{[PDB \textgreater{} Threshold]}$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
mark repeat={4},
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=mycolor1, line width=1.0pt]
  table[row sep=crcr]{%
0	1\\
0.01	0.972786\\
0.02	0.884589000000001\\
0.03	0.819929999999999\\
0.04	0.773557000000001\\
0.05	0.739119\\
0.06	0.711574000000001\\
0.07	0.688482\\
0.08	0.669480000000001\\
0.09	0.652462\\
0.1	0.638155\\
0.11	0.624554\\
0.12	0.612954\\
0.13	0.602229\\
0.14	0.592523\\
0.15	0.583056\\
0.16	0.574781\\
0.17	0.566627\\
0.18	0.559573\\
0.19	0.552757\\
0.2	0.546232\\
0.21	0.539948\\
0.22	0.534618\\
0.23	0.528986\\
0.24	0.5239\\
0.25	0.518263\\
0.26	0.513334\\
0.27	0.509089\\
0.28	0.504506\\
0.29	0.499719\\
0.3	0.496461\\
0.31	0.492155\\
0.32	0.488690000000001\\
0.33	0.484353\\
0.34	0.480905\\
0.35	0.477725\\
0.36	0.474548\\
0.37	0.470846\\
0.38	0.467968\\
0.39	0.464802\\
0.4	0.461728\\
0.41	0.458656\\
0.42	0.455989999999999\\
0.43	0.4534\\
0.44	0.45051\\
0.45	0.447786\\
0.46	0.445502000000001\\
0.47	0.442898\\
0.48	0.440171\\
0.49	0.437927\\
0.5	0.435667\\
0.51	0.432796\\
0.52	0.430816\\
0.53	0.428758999999999\\
0.54	0.426392\\
0.55	0.42451\\
0.56	0.422221\\
0.57	0.419654\\
0.58	0.417849\\
0.59	0.416263999999999\\
0.6	0.414099\\
0.61	0.412511\\
0.62	0.409804\\
0.63	0.40874\\
0.64	0.406275\\
0.65	0.404696\\
0.66	0.402639\\
0.67	0.401339\\
0.68	0.399524999999999\\
0.69	0.397724\\
0.7	0.395963\\
0.71	0.394738\\
0.72	0.392826\\
0.73	0.391512\\
0.74	0.390033\\
0.75	0.388842\\
0.76	0.386652\\
0.77	0.385205\\
0.78	0.384061\\
0.79	0.382535999999999\\
0.8	0.380781\\
0.81	0.379606999999999\\
0.82	0.377741\\
0.83	0.376568\\
0.84	0.375454999999999\\
0.85	0.37394\\
0.86	0.372341\\
0.87	0.371168\\
0.88	0.369721999999999\\
0.89	0.368764999999999\\
0.9	0.366777\\
0.91	0.365737\\
0.92	0.364814\\
0.93	0.363701\\
0.94	0.362065\\
0.95	0.361286\\
0.96	0.360002\\
0.97	0.358823\\
0.98	0.357600999999999\\
0.99	0.356438\\
1	0.355226\\
};
\addlegendentry{$\text{Max. RSRP (}\omega\text{ = 2)}$}

\addplot [color=mycolor2, line width=1.0pt]
  table[row sep=crcr]{%
0	1\\
0.01	0.972786\\
0.02	0.882520000000001\\
0.03	0.814032999999999\\
0.04	0.764644000000001\\
0.05	0.727556\\
0.06	0.697915000000001\\
0.07	0.672957000000001\\
0.08	0.652227\\
0.09	0.633859\\
0.1	0.618014\\
0.11	0.603532\\
0.12	0.590749\\
0.13	0.578993\\
0.14	0.568569\\
0.15	0.557954\\
0.16	0.548866\\
0.17	0.540005\\
0.18	0.532104\\
0.19	0.524687\\
0.2	0.517153999999999\\
0.21	0.510501\\
0.22	0.504444\\
0.23	0.498202\\
0.24	0.492311\\
0.25	0.486323\\
0.26	0.480665\\
0.27	0.475992\\
0.28	0.470899\\
0.29	0.465941\\
0.3	0.462147\\
0.31	0.457486\\
0.32	0.453394\\
0.33	0.448669\\
0.34	0.445076\\
0.35	0.441136\\
0.36	0.437737\\
0.37	0.433622\\
0.38	0.430432\\
0.39	0.427043000000001\\
0.4	0.42392\\
0.41	0.420332\\
0.42	0.417209999999999\\
0.43	0.414327\\
0.44	0.411288\\
0.45	0.408169\\
0.46	0.405439000000001\\
0.47	0.402731\\
0.48	0.399622\\
0.49	0.397392\\
0.5	0.394828\\
0.51	0.391759\\
0.52	0.389328\\
0.53	0.387071\\
0.54	0.384684\\
0.55	0.382505\\
0.56	0.380301\\
0.57	0.377231\\
0.58	0.375294\\
0.59	0.373288999999999\\
0.6	0.371077\\
0.61	0.369608\\
0.62	0.366485\\
0.63	0.365417\\
0.64	0.362573\\
0.65	0.360668\\
0.66	0.358762\\
0.67	0.357277\\
0.68	0.355260999999999\\
0.69	0.353462\\
0.7	0.351615\\
0.71	0.349967\\
0.72	0.348012\\
0.73	0.346437\\
0.74	0.344848\\
0.75	0.343509\\
0.76	0.341308\\
0.77	0.339841\\
0.78	0.338556\\
0.79	0.336613999999999\\
0.8	0.335174\\
0.81	0.333799999999999\\
0.82	0.331609\\
0.83	0.330278\\
0.84	0.329013999999999\\
0.85	0.327565\\
0.86	0.325775\\
0.87	0.324732\\
0.88	0.323019\\
0.89	0.322061999999999\\
0.9	0.320072\\
0.91	0.318793\\
0.92	0.317933\\
0.93	0.316483999999999\\
0.94	0.315003\\
0.95	0.314013\\
0.96	0.312749\\
0.97	0.311269\\
0.98	0.310116999999999\\
0.99	0.308865\\
1	0.307622999999999\\
};
\addlegendentry{$\text{Max. MEC (}\omega\text{ = 2)}$}

\addplot [color=mycolor1, dashed, line width=1.0pt, mark size=2.0pt, mark=o, mark options={solid, mycolor1}]
  table[row sep=crcr]{%
0	1\\
0.01	0.971915\\
0.02	0.892566\\
0.03	0.832309\\
0.04	0.789729\\
0.05	0.757514000000001\\
0.06	0.73241\\
0.07	0.711459000000001\\
0.08	0.693303000000001\\
0.09	0.678628000000001\\
0.1	0.664556999999999\\
0.11	0.652422000000001\\
0.12	0.641854\\
0.13	0.631562000000001\\
0.14	0.622277000000001\\
0.15	0.61345\\
0.16	0.605319\\
0.17	0.598038\\
0.18	0.590894\\
0.19	0.584500999999999\\
0.2	0.57846\\
0.21	0.57221\\
0.22	0.566511\\
0.23	0.561137\\
0.24	0.556081\\
0.25	0.551081999999999\\
0.26	0.546359\\
0.27	0.541269\\
0.28	0.537291\\
0.29	0.532839\\
0.3	0.529095\\
0.31	0.52493\\
0.32	0.521162\\
0.33	0.517338\\
0.34	0.514071\\
0.35	0.510334\\
0.36	0.506752\\
0.37	0.504082\\
0.38	0.500244\\
0.39	0.497976\\
0.4	0.495003\\
0.41	0.491503\\
0.42	0.488625000000001\\
0.43	0.485966\\
0.44	0.483378\\
0.45	0.480476\\
0.46	0.47817\\
0.47	0.474955\\
0.48	0.472797\\
0.49	0.470214\\
0.5	0.468025\\
0.51	0.465915000000001\\
0.52	0.463334\\
0.53	0.461134\\
0.54	0.458636\\
0.55	0.456846999999999\\
0.56	0.454539\\
0.57	0.452405\\
0.58	0.449396\\
0.59	0.448453\\
0.6	0.446235999999999\\
0.61	0.444581\\
0.62	0.442753\\
0.63	0.440382\\
0.64	0.439253\\
0.65	0.43685\\
0.66	0.435398\\
0.67	0.43358\\
0.68	0.431798\\
0.69	0.429052\\
0.7	0.427911\\
0.71	0.426583999999999\\
0.72	0.424775\\
0.73	0.423233\\
0.74	0.421385\\
0.75	0.420348\\
0.76	0.418498\\
0.77	0.416451\\
0.78	0.415947\\
0.79	0.414039\\
0.8	0.41217\\
0.81	0.410914\\
0.82	0.409932999999999\\
0.83	0.408274\\
0.84	0.406721999999999\\
0.85	0.405577\\
0.86	0.404108\\
0.87	0.402322000000001\\
0.88	0.401292\\
0.89	0.400148\\
0.9	0.397981\\
0.91	0.397265999999999\\
0.92	0.396134\\
0.93	0.394961999999999\\
0.94	0.393386\\
0.95	0.392511999999999\\
0.96	0.390867\\
0.97	0.390068\\
0.98	0.389136\\
0.99	0.387395\\
1	0.38621\\
};
\addlegendentry{$\text{Max. RSRP (}\omega\text{ = 10)}$}

\addplot [color=mycolor2, dashed, line width=1.0pt, mark size=2.0pt, mark=o, mark options={solid, mycolor2}]
  table[row sep=crcr]{%
0	1\\
0.01	0.971909\\
0.02	0.888812\\
0.03	0.821997\\
0.04	0.772717000000001\\
0.05	0.734376000000001\\
0.06	0.70361\\
0.07	0.677700000000001\\
0.08	0.654677\\
0.09	0.635755\\
0.1	0.617955\\
0.11	0.602004\\
0.12	0.587877\\
0.13	0.574437\\
0.14	0.562192000000001\\
0.15	0.550241\\
0.16	0.539593\\
0.17	0.530105\\
0.18	0.520416\\
0.19	0.511391999999999\\
0.2	0.503126\\
0.21	0.494792\\
0.22	0.487114\\
0.23	0.480066\\
0.24	0.472591000000001\\
0.25	0.466000999999999\\
0.26	0.459573\\
0.27	0.453131\\
0.28	0.447355\\
0.29	0.441814\\
0.3	0.435786\\
0.31	0.430683\\
0.32	0.42567\\
0.33	0.420429\\
0.34	0.415786\\
0.35	0.410374\\
0.36	0.406192\\
0.37	0.40176\\
0.38	0.397197\\
0.39	0.393845\\
0.4	0.389169\\
0.41	0.385176\\
0.42	0.380788\\
0.43	0.377551\\
0.44	0.373765\\
0.45	0.369978\\
0.46	0.367014\\
0.47	0.362443\\
0.48	0.359593\\
0.49	0.356752\\
0.5	0.353262\\
0.51	0.350296\\
0.52	0.347121\\
0.53	0.344115\\
0.54	0.340959\\
0.55	0.338448\\
0.56	0.335469\\
0.57	0.332416\\
0.58	0.329019\\
0.59	0.327418\\
0.6	0.324449\\
0.61	0.322325\\
0.62	0.320185999999999\\
0.63	0.317165\\
0.64	0.315304\\
0.65	0.312484\\
0.66	0.310505\\
0.67	0.307649\\
0.68	0.305506\\
0.69	0.303015\\
0.7	0.300792\\
0.71	0.298932\\
0.72	0.29677\\
0.73	0.294785\\
0.74	0.293097\\
0.75	0.290997\\
0.76	0.288705\\
0.77	0.286676\\
0.78	0.285581\\
0.79	0.283116\\
0.8	0.28122\\
0.81	0.278735\\
0.82	0.27794\\
0.83	0.275927\\
0.84	0.273851\\
0.85	0.272135\\
0.86	0.270918\\
0.87	0.268429\\
0.88	0.267144\\
0.89	0.265730000000001\\
0.9	0.263451\\
0.91	0.262414\\
0.92	0.260918\\
0.93	0.259534\\
0.94	0.257665\\
0.95	0.256388\\
0.96	0.254458\\
0.97	0.253787\\
0.98	0.252285\\
0.99	0.250692\\
1	0.249048\\
};
\addlegendentry{$\text{Max. MEC (}\omega\text{ = 10)}$}
\end{axis}
\end{tikzpicture}%
}
